Undirected Graphs of Entanglement Two

Entanglement is a complexity measure of directed graphs that origins in fixed point theory. This measure has shown its use in designing efficient algorithms to verify logical properties of transition systems. We are interested in the problem of deciding whether a graph has entanglement at most k. As this measure is defined by means of games, game theoretic ideas naturally lead to design polynomial algorithms that, for fixed k, decide the problem. Known characterizations of directed graphs of entanglement at most 1 lead, for k = 1, to design even faster algorithms. In this paper we present an explicit characterization of undirected graphs of entanglement at most 2. With such a characterization at hand, we devise a linear time algorithm to decide whether an undirected graph has this property.

==> algorithm_old.tex <==
\section{A Linear Time  Algorithm}
In this section we present a linear time algorithm that decides
whether a connected undirected graph $G$ has entanglement at most
$2$. As we shall see, the algorithm essentially depends on the fact
that we can test whether a graph $G$ contains a long cycle in time
$O(\card{V_{G}})$. It is then immediate to argue that there exists a
linear time algorithm to test whether an undirected graph has
entanglement at most $2$. To this goal, observe first that the tree
width of a graph satisfying condition \eqref{cond:shortcycles} is at
most $3$, by \cite{birmele}.  Considering that conditions
\eqref{cond:no3colls} and \eqref{cond:noadjcolls} are expressible in
first order logic, it is then possible to use Courcelle's Theorem
\cite[\S 6.3]{courcelle2} to argue that \eqref{cond:no3colls} and
\eqref{cond:noadjcolls} can be verified in linear time on graphs with
no long cycles.

An algorithm LONG-CYCLE-IN($G$) that detects whether $G$ has some long
cycle -- where long means here strictly longer than a fixed $k$ -- is
obtained by modifying the standard algorithm to detect cycles by
Deep-First-Search as follows.  An array $\delta$ keeps track of the
distances of nodes $v$ from the root in the DFS tree, the value
$\delta(v)$ being computed as soon as the vertex $v$ is discovered. As
soon as a back edge $(d,a)$ (i.e. $d$ is being visited and $a$ is
already visited) is discovered, the value $\delta(d)- \delta(a) + 1$
is computed. If this number is greater than $k$ then a long cycle has
been detected, the algorithm halts and accepts. Otherwise it continues
as usual in a DFS and rejects if all the edges have been explored.
Since a graph $G$ with no long cycles has at most $(k +1)\card{V} -1$
undirected edges, the algorithm LONG-CYCLE-IN($G$) runs in time
$O(\card{V_{G}})$.


The algorithm we present in the following is suggested by Theorem
\ref{zeta2alg}, stating that $\Ent{G} \leq 2$ if and only if $G \in
\zeta_{2}$.  The algorithm takes as inputs connected graphs but it is
straightforward to modify it to consider graphs that are not
necessarily connected.

% belongs to the class $\zeta_2$. Our algorithm is largely
% inspired by the proof of Proposition \ref{zeta2algonly}.  The algorithm first checks whether $G$ has a long cycle.
% If this is not the case, then it chooses a glue point candidate. One
% can remark that, at the beginning of the algorithm, a vertex of degree
% greater than $3$ may be a first candidate glue point. If such vertex
% does not exist then $G$ is a path or a cycle of length at most $4$,
% and therefore it belongs to $\zeta_2$. Once a glue point candidate $v$
% is fixed, the aim of the algorithm is to verify that each connected
% subgraph collapsed on $v$ belongs to $\zeta_2$.  Technically, we find
% all the molecules collapsed on $v$, this allows to find all the
% successor glue points of $v$. To find all the molecules around a glue
% point $v$, we explore all vertices that are at distance at most $2$
% from $v$. It is a matter of technique to isolate a molecule from those
% vertices, and to verify that conditions (\ref{cond:no3colls}) and
% (\ref{cond:noadjcolls}) are respected in that molecule.

\lstset{
  morekeywords={Procedure,Function,%
    if,then,else,begin,end,for,foreach,do,done,and,%
    otherwise, %%
    %%Input,
    return,
    accept, reject,
  },
  morecomment=[l][itshape]{//},
  mathescape=true,
  xleftmargin=8mm,
  %%frame=single,
  %%framexleftmargin=0mm
  numbers=left
}

\small
\begin{lstlisting}[]
ENTANGLEMENT-TWO($G$) 
// Input an undirected connected graph $G$, accept if $G \in \zeta_2$
if LONG-CYCLE-IN($G$) then reject 
foreach $v \in V_{G}$ 
  do color($v$) <-  Not_Visited
     ${\cal I}$_type($v$) <- Not_Affected
     $\deg[G]{v}$ <- $\card{vE}$
$v_0$ <- a vertex s.t. $\deg[G]{v_0}\neq 2$ 
if $v_0$ = Not_Found then accept 
VISIT($v_0$)
accept           
\end{lstlisting}

\begin{lstlisting}
VISIT($v$)
color(v) <- Visited
$N$ <- NEXT-GLUE-POINTS($v$)
foreach $x \in N$
  do VISIT($x$)
return
\end{lstlisting}
\normalsize %
The algorithm is similar to a DFS that explores and constructs on the
fly the graph $\derived G$ mentioned within Proposition
\ref{prop:derived}. A main difference is that the algorithm
immediately tests whether $G$ has long cycles.  If the test fails,
then $G$ is sparse, the size of $E_{G}$ being linear in $V_{G}$, and
neighbors of a glue point in the graph $\derived G$ can be computed
efficiently. The algorithm begins by choosing a vertex that
necessarily has to be a glue point of $G$ provided $G \in \zeta_{2}$.
If such a vertex is not found, then the graph $G$ is a cycle of length
at most $4$, and the algorithm accepts. The computation of the
neighbors in the graph $\partial G$ is performed by the the function
NEXT-GLUE-POINTS which also verifies that the subgraph of $G$, rooted
at $v$, connected to $v$, and not yet explored, is a collapse on $v$
of graphs of the form $\theta^{\varepsilon,n}_{v,w}\collapse{w} H$.
The proof of Lemma \ref{lemma:induct1} shows that if $\varepsilon + n
> 0$, then a graph of the form
$\theta^{\varepsilon,n}_{v,w}\collapse{w} H$ belongs to $\zeta_{2}$
if and only if $H$ belongs to $\zeta_{2}$ with $w$ a glue point of
$H$. Thus the Lemma ensures that the algorithm is sound and correct.
%%

%%
The implementation of the function NEXT-GLUE-POINTS relies on the
following considerations.  Let $G$ be a graph sastisfying
\eqref{cond:shortcycles}, $v \in V_{G}$, and denote by $xE^{v}$ the
set $\set{y \in xE\,|\,y \neq v}$.  If $x \in vE$ and $\deg[G]{x} =
2$, let $s(x)$ be the unique $y \in xE^{v}$ and $S_{2} =
\set{s(x)\,|\,x \in vE \text{ and } \deg[G]{x} = 2}$.  Let $S_{n2} =
\set{x\,|\,x \in vE \text{ and } \deg[G]{x} \neq 2} \setminus S_{2}$.
Let ${\cal I}$ be the family of subsets $\set{S_{2},S_{n2}} \cup
\set{xE^{v}\,|\,x \in S_{n2}}$, and observe that $S_{2} \cap S_{n2} =
\emptyset$ by definition.
\begin{lemma}
  \label{lemma:nextglues}
  A graph $G$ sastisfying \eqref{cond:shortcycles} is of the form
  %$\collapse{v} \theta^{\varepsilon,n}_{v,x} \collapse{x} H_{x}$ 
  $$
  (\theta^{\varepsilon_{1},n_{1}}_{v,x_{1}} \collapse{x_{1}}
  H_{1}) \collapse{v} \ldots \collapse{v}
  (\theta^{\varepsilon_{h},n_{h}}_{v,x_{h}} \collapse{x_{h}}
  H_{h})
  $$
  if and only if $A \cap B = \emptyset$, for each pair $A,B \in {\cal
    I}$, $A \neq B$.
\end{lemma}
%%
\small
\begin{lstlisting}[mathescape] 
NEXT-GLUE-POINTS($v$) 
glue_points <- $\emptyset$
foreach $x \in vE$
  do ${\cal I}$_type($x$) <- Not_Affected
foreach $x \in vE$
  do if color($x$) = Not_Visited and $\deg[G]{x} = 2$
     then color($x$) <- Visited
          foreach $y \in xE$ 
            do if $y \neq v$ and ${\cal I}$_type($y$) = Not_Affected
               then ${\cal I}$_type($y$) <- $S_{2}$ 
                    glue_points <- glue_points $\cup$ $\set{y}$
foreach $x \in vE$
  do if color($x$) = Not_Visited and $\deg[G]{x} \neq 2$ 
        and ${\cal I}$_type($x$) $\neq$ $S_{2}$
     then if ${\cal I}$_type($x$) $\neq$ Not_Affected then reject
          ${\cal I}$_type($x$) <- $S_{n2}$
          foreach $y \in xE$
          do if color($x$) = Not_Visited
             then if ${\cal I}$_type($y$) $\neq$ Not_Affected then reject
                  ${\cal I}$_type($y$) <- $N_{S_{n2}}$
          glue_points <- glue_points $\cup$ $\set{x}$
return glue_points
\end{lstlisting}
\normalsize %%
We leave the reader to verify that the algorithm visits the adjacency
list of each vertex a bounded numbers of times. In view of the fact
that if a graph $G$ satisfies \eqref{cond:shortcycles} then
$\card{E_{G}} \leq 5\card{V_{G}}$, we can therefore state:
\spnewtheorem*{fact}{Fact}{\bfseries}{\itshape}
\begin{fact}
  Algorithm ENTANGLEMENT-TWO($G$) runs in time $O(\card{V_{G}})$.
\end{fact}
Finally, we add a remark on the tree width of undirected graphs in the
class $\zeta_{2}$. The reader may have noticed that graphs in
$\zeta_{2}$ have tree width at most $2$. However, in view of
\cite[Proposition 8]{berwanger}, not every graph of tree width $2$ has
entanglement $2$: in particular the tree width of the graph 3C is $2$,
its entanglement is $3$.

 %%% Local Variables: 
 %%% mode: latex
 %%% TeX-master: "main"
 %%% End:  


==> algorithm_old_old.tex <==
\section{The algorithm}
In this section we present a linear time algorithm that decides
whether a given undirected connected graph $G$ has entanglement at
most $2$.  By Theorem \ref{zeta2alg} this is equivalent to verifying
that $G$ belongs to the class $\zeta_2$. Our algorithm is largely
inspired by the proof of Proposition \ref{zeta2algonly}. We illustrate
the algorithm on undirected connected graphs.  It is a straightforward
task to modify the algorithm to consider graphs that are not
connected. The algorithm first checks whether $G$ has a long cycle.
If this is not the case, then it chooses a glue point candidate. One
can remark that, at the beginning of the algorithm, a vertex of degree
greater than $3$ may be a first candidate glue point. If such vertex
does not exist then $G$ is a path or a cycle of length at most $4$,
and therefore it belongs to $\zeta_2$. Once a glue point candidate $v$
is fixed, the aim of the algorithm is to verify that each connected
subgraph collapsed on $v$ belongs to $\zeta_2$.  Technically, we find
all the molecules collapsed on $v$, this allows to find all the
successor glue points of $v$. To find all the molecules around a glue
point $v$, we explore all vertices that are at distance at most $2$
from $v$. It is a matter of technique to isolate a molecule from those
vertices, and to verify that conditions (\ref{cond:no3colls}) and
(\ref{cond:noadjcolls}) are respected in that molecule.
\marginpar{sur la coloration}

\lstset{
  morekeywords={Procedure,Function,%
    if,then,else,begin,end,for,foreach,do,done,%
    otherwise, %%
    %%Input,
    accept, reject,
  },
  morecomment=[l][itshape]{//},
  mathescape=true,
  frame=single,
  framexleftmargin=0mm
}

\small
\begin{lstlisting}[]
Entanglement_Two($G$) 
// Input an undirected connected graph $G$, accept if $G \in \zeta_2$
if Long_Cycle_In($G$) then reject 
foreach $v \in V_{G}$ 
  do color($v$) <-  Not_Visited
$v_0$ <- a vertex s.t. $\deg[G]{v_0}\ge 3$ 
if $v_0$ = Not_Found then accept 
color($v_0$) <-  Visited 
Solve($G,v_0$)           
\end{lstlisting}

\begin{lstlisting}
Solve($G,v$)
$D_{v}$ <- all vertices $v'$ s.t. color($v'$) = Not_Visited  
           at distance at most $2$ from  $v$
if $D_{v} = \emptyset$ then accept
$\set{D_{i}}_{i \in I}$ <- a partition of the subgraph induced by $D_{v}$ 
     into maximal connected component 
foreach $i \in I$
  do  $v_i$ <- Next_Glue_Point($D_{i},v$)
      if $v_{i}$ = Not_Found then reject 
      Solve($G,v_i$)
accept
\end{lstlisting}
\newpage
\normalsize 
\small
\begin{lstlisting}[mathescape] 
Next_Glue_Points($v$) 
ret <- $\emptyset$

foreach $v' \in N$
  do color($v'$) <- Visited

foreach $x \in vE$
  do if $\deg[G]{x} = 1$ 
     then ret <- ret $\cup$ $\set{x}$

foreach $x \in vE$
  do if $\deg[G]{x} = 2$ 
     then foreach $y \in xE$ 
            do if $y \neq v$ 
               then color(y) <- Red 
                    ret <- ret $\cup$ $\set{y}$

foreach $x \in vE$
  do if $\deg[G]{x} \geq 3$ 
     then if color(x) $\neq$ Red
          then foreach $y \in xE$
               do if color(y) = Red then reject
                  else color(y) <- Red
          ret <- ret $\cup$ $\set{x}$
return ret
\end{lstlisting}

\small
\begin{lstlisting}[mathescape] 
Function  Next_Glue_Point($D_{i},v$) 
// Test whether $D_{i}\cup \set{v}$ contains a molecule $\theta^{\varepsilon,n}_{v,v_i}$
// return the second glue point $v_{i}$

$N_i$ <- vertices in $D_{i}$ at distance $1$ from $v$
foreach $v' \in N_{i}$
  do color($v'$) <- Visited
if $N_i = \set{v_1}$ then return $v_1$
if $(N_i=\set{v_1,v_2})$  
  then if $\set{v_1,v_2}\in E(G)$ 
       then if $\deg[G]{v_1}>2$ and $\deg[G]{v_2}>2$ 
            then return Not_Found
            else if $\deg[G]{v_1}> \deg[G]{v_2}$ 
                 then return $v_1$
                 else return $v_2$ 
       else if $\deg[G]{v_1}>2$ or $\deg[G]{v_2}>2$ 
            then return Not_Found 
            else let $x \in D_{v_0,i} \setminus \set{v_1,v_2}$
                 color($x$) <- Visited 
                 return $x$ 
else // Assume $N_i=\set{v_1,...,v_n}$, $n \geq 3$
     if $\forall v_k \in N_i : \deg[G]{v_k}=2 $ 
     then //  we have  $\theta_{v_0,x}^{0,n}$
          let $x \in D_{v_0,i} \setminus N_i$
          color($x$) <- Visited
          return $x$ 

     if $(\exists v_k \in N_i :\deg[G]{v_k}>2)$ and $(\forall v \in N_i \setminus \set{v_k} : \deg[G]{v}=2)$ 
            and $\exists v_l \in N_i : \set{v_l,v_k} \in E(G)$ 
     then // we have $\theta_{v_0,v_k}^{1,n-1}$ 
          color($N_i$)
          return $v_k$   
return Not_Found 
\end{lstlisting}
\normalsize

Algorithm accepts if it halts and any reject exception is raised.  

\subsection{Detecting Long Cycles}

To detect long cycles, we modify the standard algorithm
\cite[???]{Algorithms} to detect
cycles in an undirected graphs by means of a depth-first search.

Let us recall that a pointed digraph $\langle V,E,v_{0} \rangle$ is a
tree if for each $v \in V$ there exists a unique path from $v_{0}$ to
$v$.
\begin{definition}
  A tree with back-edges is a tuple $\langle V,T,v_{0},B \rangle$ such
  $\langle V,T,v_{0} \rangle$ is a tree, and $B \subseteq V \times V$
  is such that if $x B y$ then $y$ is an ancestor of $x$ in the tree 
  $\langle V,T,v_{0} \rangle$.
\end{definition} 
Observe that by definition $(x,y) \in T \cap B$ implies $x = y$. For a
tree with back edge as above let $\delta(v)$ be the length of the
unique path from $v_{0}$ to $v$ on the tree. If $(d,a) \in B$ is a
back edge, then we define
\begin{align*}
  \ell(d,a) & = \delta(d) - \delta(a) + 1\,.
\end{align*}
\begin{definition}
  A TwBE representation of an undirected connected graph $G = \langle
  V,E\rangle$ is a tree with back edges of the form $\langle
  V,T,v_{0},B \rangle$, satisfying the following conditions:
  \begin{enumerate}
  \item if $\couple{a,b} \in E$, then $(a,b) \in T \cup B$ or $(b,a)
    \in T \cup B$,
  \item if $(a,b) \in  T \cup B$, then $\couple{a,b} \in E$.
  \end{enumerate}
\end{definition}
Clearly, a TwBE representation of an undirected graph is such that $T
\cap B = \emptyset$. Something more is true: if $(d,a) \in B$, then
$\ell(d,a) \geq 2$. If $\ell(d,a) = 0$ then $d = a$, but it is not the
case (by Definition) that $\set{d,d} \in E$. If $\ell(d,a) = 1$, then
$(a,d) \in T$, contradicting condition 1. Representations of this kind
are obtained by running a DFS on an undirected graph, according to the
following standard Lemma \cite{Tarjan72}.
\begin{lemma}
  Let $(V,\bar{E}_\mathcal{T})$ be a DFS tree of un undirected graph
  $(V,E)$. If an edge $\set{a,b} $ is in $E\setminus
  \bar{E}_{\mathcal{T}}$ then either $a$ is an ancestor of $b$, or $a$
  is a descendant of $b$ in $T$.
\end{lemma}


\begin{proposition}\label{cycle:bij}
  If ${\cal T} = \langle V,T,v_{0},B\rangle$ is a TWBE representation
  of an undirected graph $G = (V,E)$, then there is bijection $\psi$
  from the set of simple cycles of $G$ and back-edges of ${\cal T}$.
  The length of a simple cycle $\gamma$ being equal to
  $\ell(\psi(\gamma))$.
\end{proposition}
\begin{proof}
  Let $\gamma = a_{0}a_{1}\ldots a_{n-1}a_{n}$, $n \geq 3$, where
  $a_{n} = a_{0}$ be a simple cycle of $G$. We can assume that
  $\delta(a_{0}) \leq d(a_{i})$, for $i = 1,\ldots ,n-1$. Let
  us prove that $(a_{k-1},a_{k}) \in T$ for $k = 1,\ldots ,n-1$. Let
  us suppose that $(a_{i-1},a_{i}) \in T$ for $i < k$.  If
  $(a_{k-1},a_{k}) \in B$, then $a_{k}$ is an ancestor of $a_{k-1}$,
  i.e. it lies on the path from $v_{0}$ to $a_{k-1}$. This directed
  path has the form $v_{0}\ldots v'a_{0}a_{1}\ldots a_{k-1}$, hence we
  have three possibilities. (i) $a_{k}$ belongs to the interval
  $v_{0}\ldots v'$: this is not possible, otherwise $\delta(a_{k}) <
  \delta(a_{0})$.  (ii) $a_{k}$ belongs to the interval $a_{1}\ldots
  a_{k-2}$: this is not possible, since otherwise the cycle is not
  simple. (iii) $a_{k} = a_{0}$, but, as before, this is only possible
  if $k = n$. Thus we define $\psi(\gamma) = (a_{n-1},a_{0})$ where
  $\delta(a_{0})$ is minimal.
  
  Clearly such a correspondence has an inverse: each back edge $(d,a)
  \in B$ lies on a direcetd cycle $aT\ldots TdBa$ in the graph $(V,T
  \cup B)$ of length at least $3$. Since $G$ is the symetrization of
  $(V,T \cup B)$, the direcetd cycle $aT\ldots TdBa$ gives rise to the
  undirected cycle $\psi^{-1}(d,a) = aE\ldots EdEa$.
\end{proof}

An algorithm to detect long cycles -- where long means here strictly
longer than a given $k$ -- in an undirected graph $G$ can be obtained
from a DFS according to the following modifications. An array keeps
track of $\delta(v)$ for $v \in V$, which are computed as soon as a
the vertex $v$ is visited first. As soon an edge of the form $(a,b)$
with $d$ the current vertex and $a$ already visited (i.e. if a back
edge is found or if $a$ is the father of $d$) then $\delta(d)-
\delta(a) + 1$ is computed. If this number is greater than $k$ then
the algorithm halts and rejects. Otherwise it continues as usual in a
DFS.  It accepts if it does not halt because a long cyle has been
detected.
\begin{lemma}
  A tree with back edges such that $0 < \ell(d,a) \leq k$ for each
  back edge $(d,a)$ has at most $(k +1)\card{V} -1$ egdes.
\end{lemma}
\begin{proof}
  The edges from $T$ are as usual $|V|-1$. Every vertex $d$ can be the
  source of at most $k$ back edges. Hence we obtain
  \begin{align*}
    \card{T \cup B}
     = \card{T} + \card{B}
    & \leq (\card{V}-1) + k\card{V}
    = (k +1)\card{V} -1\,.
  \end{align*}
\end{proof}
The lamma above clerly shows that the proposed to detect long cycles
runs in time linear in $\card{V}$, for a fixed $k$.




Now we show that depth-first search (DFS briefly) techniques allow us
to detect a long cycle. The DFS strategy is to scan the graph as deep
as possible such that all edges must be traversed once. In this
technique, edges are explored out of the most recently discovered
vertex $v$ that still has unexplored edges leaving it. When all of
$v'$s edges have been explored, the search backtracks to explore edges
leaving the vertex from which $v$ was discovered. After applying DFS
to an undirected graph $(G,E)$ let us consider the set of edges
$E_\mathcal{T}$ consisting of all edges of the form $(v_i,v_j)$ such
that the vertex $v_j$ has been discovered from $v_i$. the digraph
$(V,E_\mathcal{T})$ is called the \textbf{DFS tree}. This name is due
to the following observation \cite{Shimeon}: the digraph
$(V,E_{\mathcal{T}})$ defined above is a directed tree.  The following
usefull lemma is due to \cite{Hop73}, \cite{Tarj:72}:
\begin{lemma}
Let $(V,\bar{E}_\mathcal{T})$ be the undirected version of a DFS tree $T$, of $G(V,E)$. If an edge $\set{a,b} $ is in $E\setminus \bar{E}_{\mathcal{T}}$ then either $a$ is an ancestor of $b$, or $a$ is a descendant of $b$ in $T$.  
\end{lemma}
In other words the previous lemma states that every non-tree edge connects some vertex back to one of its ancestors, thus we can define a DFS tree with back-edges as follows:
\begin{definition}[\textbf{DFS tree with back-edges}]
 Let $G=(V,E)$ be an undirected graph,  $(V,E_{\mathcal{T}})$ its DFS directed tree, and $(V,\bar{E}_{\mathcal{T}})$ the related undirected DFS tree. The DFS tree with back-edges of $G$ is $(V,E_{\mathcal{T}}\cup E_{\mathcal{B}})$ such that $(b,a) \in E_{\mathcal{B}}$ if and only if $\set{a,b} \in E \setminus \bar{E}_{\mathcal{T}} $ and $a$ is an ancestor of $b$ in  $(V,E_{\mathcal{T}})$. 
\end{definition} 
 
\begin{corollary}\label{edge:part}
  If $T=(V,E_{\mathcal{T}}\cup E_{\mathcal{B}})$ is a DFS tree with
  back-edges of an undirected graph $G=(V,E)$, then whenever
  $\set{a,b} \in E$ then we have exclusively either $(a,b) \in
  E_\mathcal{T}$ or $(a,b) \in E_\mathcal{B}$ or $(b,a) \in
  E_\mathcal{T}$ or $(b,a) \in E_\mathcal{B}$.
\end{corollary} 

Now we describe  the function that detects a long cycle in an undirected graph $G$. We label each discovered vertex $v$ in DFS by its distance $d(v)$ from the root, since there is a bijection between simple cycles of $G$ and the related DFS tree with back-edges, we can compute on the fly the length of every  cycle each time a back-edge $(v_i,v_j)$ is created in DFS, the length of such cycle in nothing than $d(v_i)-d(v_j)+1$. \marginpar{un mot sur les back-edges triviaux????}  


\subsection{Completeness}
  The following lemma is the key by which the induction in the proof of proposition \ref{comp:prop} works.
 \begin{lemma}\label{comp:induc}
  Let $G_1,G_2 \in \zeta_2$ and $G=G_1 \overline{\bigoplus}_{v} G_2$. If the algorithm accepts $G_1$ and $G_2$ then it accepts $G$.
 \end{lemma} 
 \begin{proof}
 Assume that we launch the algorithm from $v_1 \in V(G_1)$. Since $v$ is a glue point, it will be recognised by the algorithm as a glue point candidate. So when it meets it, it continues to explore the branche $G_2$, and hence accepts it, since the branche $G_1$ is cleary accepted.
 \end{proof}
 \begin{proposition}\label{comp:prop}
  The algorithm described above is complete i.e. if $G \in \zeta_2$ then the algorithm accepts it.
 \end{proposition}
 \begin{proof}
 The proof is by induction on $|V(G)|$. Clearly the Proposition holds for every molecule and the neutral graph $\eta$. Let us assume that it holds for all graphs $H$ such that $|V(H)|  \le |V(G)|$.  
First note that any connected graph $G \in \zeta_2$ is of the form  
 $$ G= G_1 \overline{\bigoplus}_{v_1} \theta_{v_1,v_2}^{\varepsilon,n} \overline{\bigoplus}_{v_2} G_2 $$ 
Where $\varepsilon+n > 0$ and $G_1,G_2$ are connected, eventually empty, graphs in $\zeta_2$. 
Hypothesis induction implies that the algorithm accepts $G_1$ and $G_2$, thus from lemma \ref{comp:induc} it accepts $G_1 \overline{\bigoplus}_{v_1} \theta_{v_1,v_2}^{\varepsilon,n}$, and hence  accepts $\big ( G_1 \overline{\bigoplus}_{v_1} \theta_{v_1,v_2}^{\varepsilon,n} \big) \overline{\bigoplus}_{v_2} G_2$.  
 
 \end{proof}
 
\subsection{Soundness}
The following two lemmas show that the constraints imposed by function $Check\_molecule$ on the degree of vertices in $D_{v_0,i}$ are sufficient to verify that the graph induced by  $D_{v_0,i}\cup \set{v_0}$ contains a molecule.

Let $G_{v_0}$ be a connected undirected graph such that $v_0 \in V(G_{v_0})$, $G_{v_0} \setminus \set{v_0}$ is connected, and all simple cycle of $G_{v_0}$ are short, moreover all vertices are at distance at most $2$ from $v_0$. We denote by $N_{v_0}$ the vertices at distance $1$ from $v_0$. If $|N_{v_0}|\ge 3 $, then  we have the  following lemmas:

\begin{lemma}\label{sound1}
  If $\forall v \in N_{v_0}: \deg[G_{v_0}]{v}=2$ then $G_{v_0}$ is a molecule $\theta_{v_0,v_x}^{0,|N_{v_0}|}$ with $V(G_{v_0})\setminus (N_{v_0}\cup \set{v_0})=\set{v_x}$
\end{lemma}
\begin{proof}
Note first that $\forall v_i,v_j \in N_{v_0}$ we have $\set{v_i,v_j} \notin E(G_{v_0})$, otherwise assume that $v_1,v_2,v_i \in N_{v_0}$ and $\set{v_1,v_2} \in E(G_{v_0})$. Since $G_{v_0}\setminus\set{v_0}$ is connected, there is a path in  $G_{v_0}\setminus\set{v_0}$ from $v_i$ to both $v_1$ and $v_2$, which implies $\deg[G_{v_0}]{v_1} > 2$  or $\deg[G_{v_0}]{v_2} > 2$, absurd. Since vertices in $N_{v_0}$ have degree $2$ and all vertices in $G_{v_0}$ are at distance at most $2$ from $v_0$, so $\forall v_i, v_j \in N_{v_0} : \exists ! x_{i,j} \in G_{v_0} \setminus N_{v_0} \cup \set{v_0}$ such that $\set{v_i,x_{i,j}},\set{v_j,x_{i,j}} \in E(G_{v_0})$. Also there must exist a path from each $x_{p,q}$ to $x_{i,j}$. (\ref{cond:shortcycles}) condition implies that $x_{i,j}=x_{p,q}$, for all $i,j,p,q$. Thus $G_{v_0}$ is a molecule $\theta_{v_0,x_{i,j}}^{0,|N_{v_0}|}$. 
 
 \end{proof}

\begin{lemma} \label{sound2}
 If $ \exists v_k \in N_{v_0} : \deg[G_{v_0}]{v_k}>2 $ , $ \forall v \in N_{v_0} \setminus \set{v_k} : \deg[G_{v_0}]{v}=2$ and $\exists v_m \in N_i: \set{v_m,v_k} \in E(G_{v_0})$,  then the graph induced by $N_{v_0} \cup \set{v_0}$ is a molecule $\theta_{v_0,v_k}^{1,|N_{v_0}|-1}$. 
\end{lemma}
\begin{proof}
  Let us denote by $N_{v_k}$ the vertices at distance $1$ from $v_k$ in $V(G_{v_0})\setminus (N_{v_0} \cup \set{v_0})$. We shall prove that $\forall v_i \in N_{v_0}\setminus \set{v_k}:$ $\set{v_i,v_k} \in E(G_{v_0})$.  First note that $\forall v_i,v_j \in N_{v_0}\setminus\set{v_k} : \set{v_i,v_j} \notin E(G_{v_0})$ for the same reason mentioned in the proof of lemma \ref{sound1}. Let $v_i \in N_{v_0}\setminus \set{v_k,v_m}$, since $\deg[G]{v_i}=2$ and the graph induced by $G_{v_0}\setminus\set{v_0}$ is connected we have either $\set{v_i,v_k} \in E(G_{v_0})$ or $\exists w_i \in N_{v_k}$ such that $\set{v_i,w_i} \in E(G_{v_0})$. We can not have the second possibility, because $v_0 v_m v_k w_i v_i v_0$ is a long cycle, therefore  $\forall v_i \in N_{v_0}\setminus \set{v_k}$ we have $\set{v_i,v_k} \in E(G_{v_0})$, so the graph induced by $N_{v_0} \cup \set{v_0}$ is  a molecule $\theta_{v_0,v_k}^{1,|N_{v_0}|-1}$.
\end{proof}
 
\begin{proposition}
  The algorithm is sound i.e. if it accepts $G$ then $G \in \zeta_2$.
 \end{proposition}
 \begin{proof}
 Immediat from lemmas \ref{sound1}, \ref{sound2} and the proof of theorem \ref{zeta2alg}
 \end{proof}
\subsection{Time complexity}
 \begin{lemma}\label{long:cycle}
 Detecting a long cycle in an undirected graph $G=(V,E)$ runs in time $O(|V|)$.
 \end{lemma}
 \begin{proof}
 In \cite{Tremaux}, authors gives a DFS algorithm that runs in time  $O(|E|)$. The function that detects a long cycle described above should run also in $O(|E|)$. Let $T=(V,E_\mathcal{T}\cup E_\mathcal{B})$ be the DFS tree with back-edges of $G$,  and $\bar{T}=(V,\bar{E}_{\mathcal{T}})$ the undirected tree of $(V,E_{\mathcal{T}})$. First note that $E=E_{\mathcal{T}} + E_{\mathcal{B}} = \bar{E}_{\mathcal{T}} +E_{\mathcal{B}}$.

If $G$ has not a long cycle  then we claim that $|E| \le 3 |V| -1$, because $|\bar{E}_{\mathcal{T}}|= |V|-1$ and if there is a back-edge from $v_i$ to $v_j$ then $v_i$ is at distance at most $3$ from $v_j$ and at least $2$ in $\bar{T}$, thus from any vertex there out goes  at most $2$ back-edges. Therfore $|E_{\mathcal{B}}| \le 2|V|$. Hence
 $|E|= \le 3|V| -1$. We conclude that detecting a long cycle in undirected graph runs in linear time in the number of vertices.
 \end{proof}

\begin{proposition}
 Entanglement algorithm runs in linear time in the size of the graph.
\end{proposition}
 \begin{proof}
  Since detecting a long cycle and checking whether a connected component is a molecule (i.e. function $check\_molecule$) run in linear time in the size of the graph, we focus on function $solve(G,{v_i})$. Recall that function $solve$ finds all vertices at distance at most $2$ from $v_i$, noted $D_{v_i}$ and then finds all the connected component of the subgraph induced by $D_{v_i}$. It is clear that the first operation runs in $O(|V|)$. The second operation may be performed in time $O(|V|+|E|)$, see \cite{Algorithms}, by using depth-first search techniques.
We have shown that if all cycles of $G$ are short then $|V|=O(|E|)$, thus finding connected components runs in time $O(|V|)$. Finally, recursive call of function $Solve$ is performed with the remaining subgraph, since already explored vertices are colored. We conclude that entanglement algorithm runs in time $O(|V|)$.     
    
 \end{proof}
 %%% Local Variables: 
 %%% mode: latex
 %%% TeX-master: "main"
 %%% End:  


==> biconnected.tex <==
\subsection{Recognizing Molecules}

\begin{lemma}
  If a biconnected component $C$ is the singleton $\set{v}$, then $v$
  is an isolated point of $G$.
\end{lemma}
\begin{proof}
  Indeed, if $\set{v,u} \in E$, then $\set{v,u}$ is a biconnected
  subset of $G$, since every singleton graph is connected.  \qed
\end{proof}

\begin{lemma}
  If $C$ is a biconnected component of a graph $G = (V,E)$ and $v \in
  C$ is not an articulation point of $G$, then $vE \subseteq C$.
\end{lemma}
\begin{proof}
  Let us suppose that $\couple{v,u} \in E$ for some $u \in V \setminus
  C$ and prove that $v$ is an articulation point of $G$.  It is not
  possible that $C = \set{v}$ since $v$ is not isolated. Therefore
  there exists $x \in C$, $x \neq v$. If in $G$ there exists a path
  from $u$ to $x$ which does not visit $v$, then we can extend $C$ to
  a greater biconnected component to which $u$ belongs. Therefore such
  a path does not exists, and $v$ is an articulation point separating
  $u$ from $x$.  \qed
\end{proof}

\begin{lemma}
  Let $G = (V,E)$ be a biconnected graph and $D \subseteq V$ be such
  that $\set{v \in V \mid \deg{v} \neq 2} \subseteq D$.
  %%
  Then $G$ is isomorphic to a molecule, with every element of $D$ sent
  by the isomorphism to a
  glue point of the molecule, if and only if either 
  \begin{align}
    \tag{i} \label{eq:fcase}
    & \card{D} = 2 \text{ and }
    V \setminus D \subseteq dE\,, \;d \in D
    \intertext{or}
    \tag{ii}  \label{eq:scase}
    & \card{D} < 2 \text{ and } \card{V} \in \set{3,4}\,.
  \end{align}
\end{lemma}
\begin{proof}
  Let us consider a biconnected molecule $\theta^{\epsilon,n}_{a,b}$
  and observe first that: (a) $\epsilon + n > 0$ since it is connected
  and (b) $(\epsilon,n) \neq (0,1)$ since it is biconnected.  Let $D
  \subseteq \set{a,b}$ be such that $\set{v \in V \mid \deg{v} \neq 2}
  \subseteq D$: clearly $\card{D} \leq 2$.

  If $\card{D} = 2 $, then $D = \set{a,b}$ and \eqref{eq:fcase} holds.
  If $\card{D} < 2$ then $\theta^{\epsilon,n}_{a,b}$ contains at most
  one vertex of degree distinct from $2$. Since $\deg{a} = \deg{b} =
  \epsilon + n$, this implies that $\theta^{\epsilon,n}_{a,b}$
  contains no vertex of degree distinct from $2$. We have therefore
  $(\epsilon,n) = (0,2)$ and $\card{V} = 4$ or $(\epsilon,n) = (1,1)$
  and $\card{V} = 3$ so that \eqref{eq:scase} holds.


  Conversely, let us consider a biconnected graph $G = (V,E)$ and let
  $D \subseteq V$ be such that $\set{v \in V \mid \deg{v} \neq 2}
  \subseteq D$.

  Let us suppose that \eqref{eq:fcase} holds and let $D = \set{a,b}$.
  Therefore if $x \not\in D$, then $\deg{x} = 2$ and since
  $\couple{x,a},\couple{x,b} \in E$, then $\set{a,b} = xE$. We have
  therefore that $G$ is isomorphic to $\theta^{\epsilon,n}_{a,b}$
  where $n = \card{V} -2$ and $\epsilon = 1$ if $\set{a,b} \in E$ and
  otherwise $\epsilon = 0$.

  Let us suppose that \eqref{eq:scase} holds, i.e. that $\card{D} < 2$
  and $\card{V} \in \set{3,4}$. Let us assume first that $\card{V} =
  3$. By looking at the list of graphs with $3$ vertices, we observe
  that only the total graph $K_{3}$ is biconnected, hence $G$ is
  isomorphic to $\theta^{1,1}_{a,b}$.
  %%
  If $\card{V} = 4$, then we claim that every vertex of $G$ has degree
  $2$, so that $G$ is isomorphic to $\theta^{0,2}_{a,b}$.  To prove
  the claim, observe that $G$ may have at most one vertex whose degree
  is not $2$. Suppose that such a vertex exists and call it $v_{0}$,
  so that $\deg{v_{0}} \in \set{1,3}$ since $G$ is connected.
  Then the usual formula 
  \begin{align*}
    2\card{E} & = \deg{v_{0}} + \sum_{v \neq v_{0}} \deg{v}
    = \deg{v_{0}} + 6
  \end{align*}
  leads to a contradiction.  \qed
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> decomposition.tex <==
\subsection{Decomposition of Graphs in $\zeta_{2}$}
\begin{lemma}[i.e. Lemma \ref{lemma:induct1}]
  Let $G$ be an undirected graph satisfying
  \eqref{cond:no3colls} and \eqref{cond:noadjcolls}.  If $G =
  \theta_{v,b}^{\varepsilon,n} \collapse{b} H$ and $H \in \zeta_2$,
  then there is a subset $\glue' \subseteq V_{G}$ such that
  $(H,\glue')$ is a glue graph in $\zeta_{2}$, $b \in Gl'$, and
  moreover $G$ is the result of the legal collapse
  \begin{align*}
    G & = \theta_{v,b}^{\varepsilon,n} \lcollapse{b} (H,Gl)\,. 
  \end{align*}
  Consequently, $G \in \zeta_2$, with $v$ a glue point of $G$.
\end{lemma}
\begin{proof}
  Since  the graph $H$ is in $\zeta_{2}$, it already comes with a set
  of glue points $\glue_{H}$. Hence, if
  $b \in \glue_H$ then we simply let $\glue' =\glue_H$.
  
  Otherwise $b$ is a dead point of a certain molecule
  $\theta_{c,d}^{\delta,m}$ of $H$, so that we can write
  \begin{align}
    \label{eq:H}
    H & %= \theta_{c,d}^{\delta,m} \lcollapse{d} H'
    = H_{c} \lcollapse{c} \theta_{c,d}^{\delta,m} \lcollapse{d}
    H_{d}\,.
  \end{align}
  Observe also that $m \geq 1$ since $b$ is a dead point of the
  molecule $\theta_{c,d}^{\delta,m}$.

  If $\theta_{v,b}^{\varepsilon,n}$ is disconnected, i.e.
  if $\varepsilon = n = 0$, then the result is obvious, since then
  \begin{align*}
    \theta_{v,b}^{\varepsilon,n} \collapse{b} \theta_{c,d}^{\delta,m}
    \lcollapse{c} H_{c} \lcollapse{d} H_{c}
    & = \theta_{v,b}^{\varepsilon,n}
    \lcollapse[b]{b,c} \theta_{c,d}^{\delta,m}
    \lcollapse{c} H_{c} \lcollapse{d} H_{c} \,.
  \end{align*}
  
  Otherwise, if $\varepsilon + n > 0$, then $\deg[G]{b} \geq 3$, since
  $b$ has two neighbors in the molecule $\theta_{c,d}^{\delta,m}$ and
  at least one neighbor in the molecule
  $\theta_{v,b}^{\varepsilon,n}$.
  
  If $\delta = 0$ then $1 \leq m \leq 2$: condition
  \eqref{cond:noadjcolls} implies that if $m \geq 2$ then $\deg[G]{c}
  = \deg[G]{d} = 2$.  If $m = 1$, then we can use the equality
  \begin{align*}
    \theta^{0,1}_{c,d} & =
    \theta^{1,0}_{c,b} \lcollapse{b} \theta^{1,0}_{b,d}
  \end{align*}
  to add $b$ to the set of glue points of $H$.  If $m = 2$, then
  $\deg[G]{c} = \deg[G]{d} = 2$. Let $e$ be the unique dead point of
  $\theta_{c,d}^{\delta,m} = \theta_{c,d}^{0,2}$ which is distinct
  from $b$. We claim that we can replace the pair $c,d$ with
  $b,e$ in the set of glue points of $H$. As a matter of fact,
  in the algebraic expression \eqref{eq:H} the legal collapses are
  disjoint. This means that we can write
  \begin{align*}
    H_{c} & = H_{c'} \lcollapse{c'} \theta^{0,0}_{c',c} & H_{d} & =
    \theta^{0,0}_{d,d'} \lcollapse{d'} H_{d'} \,,
  \end{align*}
  and consequently we can also write
  \begin{align*}
    H &  = H_{c}
    \lcollapse{c} \theta_{c,d}^{\delta,m}
    \lcollapse{d} H_{d} \\
    & = H_{c'} \lcollapse{c'} \theta^{0,0}_{c',c}
    \lcollapse{c} \theta_{c,d}^{\delta,m}
    \lcollapse{d} 
    \theta^{0,0}_{d,d'} \collapse{d'} H_{d'}
    \\
    & = H_{c'} \lcollapse{c'} \theta^{0,0}_{c',b}
    \lcollapse{b} \theta_{b,e}^{\delta,m}
    \lcollapse{d} 
    \theta^{0,0}_{e,d'} \lcollapse{d'} H_{d'}
    \,.
  \end{align*}
%   where $e$ is the second dead point of the molecule $\theta^{c,d}$.
%   That is, we can replace $c,d$ with $b,e$ in the set of glue points of
%   $H$.


  If $\delta = 1$, then $m = 1$, since condition \eqref{cond:no3colls}
  implies either $\deg{c} = 2$ or $\deg{d} = 2$, hence $m = 1$. Let us
  suppose that $\deg{d} = 2$.  We claim that we can replace $d$ with
  $b$ in the set of glue points of $H$.

  In the algebraic
  expression \eqref{eq:H} the legal collapses on $d$ are disjoint:
  that is we can write
  \begin{align*}
    H_{d} & = \theta^{0,0}_{d,d'} \lcollapse{d'} H_{d'} \,.
  \end{align*}
  Consequently we can write
  \begin{align*}
    H &  = H_{c}
    \lcollapse{c} \theta_{c,d}^{\delta,m}
    \lcollapse{d} H_{d} \\
    & = H_{c}
    \lcollapse{c} \theta_{c,d}^{\delta,m}
    \lcollapse{d} 
    \theta^{0,0}_{d,d'} \lcollapse{d'} H_{d'}
    \\
    & = H_{c} 
    \lcollapse{c} \theta_{c,b}^{\delta,m}
    \lcollapse{d} 
    \theta^{0,0}_{b,d'} \lcollapse{d'} H_{d'}
    \,.
  \end{align*}
  \qed
%   That is, we can replace $d$ with $b$ in the set of glue points of
%   $H$.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> longcycles.tex <==

\subsection{Graphs Without  Long Cycles are Sparse}

Let us recall that a pointed digraph $\langle V,E,v_{0} \rangle$ is a
tree if for each $v \in V$ there exists a unique path from $v_{0}$ to
$v$.
\begin{definition}
  A tree with back-edges is a tuple $\langle V,T,v_{0},B \rangle$ such
  $\langle V,T,v_{0} \rangle$ is a tree, and $B \subseteq V \times V$
  is such that if $x B y$ then $y$ is an ancestor of $x$ in the tree 
  $\langle V,T,v_{0} \rangle$.
\end{definition} 
For a tree with back edge as above let $\delta(v)$ be the length of
the unique path from $v_{0}$ to $v$ on the tree. If $(d,a) \in B$ is a
back edge, then we define
\begin{align*}
  \ell(d,a) & = \delta(d) - \delta(a) + 1\,.
\end{align*}
We observe that $\ell(d,a)$ is the number of vertices on the path from
$a$ to $d$.
\begin{definition}
  A TwBE representation of an undirected connected graph $G = \langle
  V,E\rangle$ is a tree with back edges of the form $\langle
  V,T,v_{0},B \rangle$, satisfying the following conditions:
  \begin{enumerate}
  \item if $\couple{a,b} \in E$, then $(a,b) \in T \cup B$ or $(b,a)
    \in T \cup B$,
  \item $(a,b) \in T \cup B$ implies $(b,a) \not\in T \cup B$,
  \item if $(a,b) \in  T \cup B$, then $\couple{a,b} \in E$.
  \end{enumerate}
\end{definition}
% Clearly, a TwBE representation of an undirected graph is such that $T
% \cap B = \emptyset$. Something more is true: if $(d,a) \in B$, then
% $\ell(d,a) \geq 2$. If $\ell(d,a) = 0$ then $d = a$, but it is not the
% case (by Definition) that $\set{d,d} \in E$. If $\ell(d,a) = 1$, then
% $(a,d) \in T$, contradicting condition 1.
Representations of this kind are obtained by running a DFS on an
undirected graph, according to the following standard Lemma (see
\cite[Theorem 23.9]{Algorithms}).
\begin{lemma}
  Let $(V,\bar{E}_\mathcal{T})$ be a DFS tree of an undirected graph
  $(V,E)$. If an edge $\set{a,b} $ is in $E\setminus
  \bar{E}_{\mathcal{T}}$ then either $a$ is an ancestor of $b$, or $a$
  is a descendant of $b$ in $T$.
\end{lemma}

\begin{lemma}
  A $\langle V,T,v_{0},B \rangle$ tree with back edges such that $0 <
  \ell(d,a) \leq k$ for each back edge $(d,a)$ has at most $(k
  +1)\card{V} -1$ egdes. If $\langle V,T,v_{0},B \rangle$ is a TwBE
  representation of an undirected connected graph, then it has at most
  $(k -1)\card{V} -1$.
\end{lemma}
\begin{proof}
  The edges from $T$ are as usual $|V|-1$. Every vertex $d$ can be the
  source of at most $k$ back edges. Hence we obtain
  \begin{align*}
    \card{T \cup B}
     = \card{T} + \card{B}
    & \leq (\card{V}-1) + k\card{V}
    = (k +1)\card{V} -1\,.
  \end{align*}
  If moreover $\langle V,T,v_{0},B \rangle$ is the representation of
  an undirected graph, we cannot have back edges of the form $(d,d)$,
  not back edges of the form $(d,a)$ if $\ell(d,a) = 1$. Therefore
  Every vertex $d$ can be the source of at most $k-2$ back edges. The
  formula follows as before.  \qed
\end{proof}

\begin{lemma}
  Let $\langle V,T,v_{0},B \rangle$ be a TwBE representation of an
  undirected connected graph $G = \langle V,E\rangle$ whose simple
  cycles have length less than $k$. Then  for each backedge $(d,a)$ we
  have $0 < \ell(d,a) \leq k$.
\end{lemma}
\begin{proof}
  Suppose that $k < \ell(d,a)$, then the path from $a$ to $d$ together
  with the edge from $d$ to $a$ form on $G$ an undirected cycle of
  length $\ell(d,a) > k$.  \qed
\end{proof}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> searching.tex <==

\subsection{Searching the Next Glue Points}
Let $G$ be a graph sastisfying \eqref{cond:shortcycles}, let $v \in
V_{G}$, and denote by $xE^{v}$ the set $\set{y \in xE\,|\,y \neq v}$.
If $x \in vE$ and $\deg[G]{x} = 2$, let $s(x)$ be the unique $y \in
xE^{v}$. Let
\begin{align*}
  S_{2} & = \set{s(x)\,|\,x \in vE \text{ and } \deg[G]{x} =
    2}\,, \\
  S_{n2} & = \set{x\,|\,x \in vE \text{ and } \deg[G]{x} \neq
    2} \setminus S_{2}\,,\\
  {\cal I} & =\set{S_{2},S_{n2}} \cup \set{xE^{v}\,|\,x \in S_{n2}}\,.
\end{align*}
Observe that
$S_{2} \cap S_{n2} = \emptyset$ by definition.
\begin{lemma}[i.e. Lemma \ref{lemma:nextglues}]
  A graph $G$ sastisfying \eqref{cond:shortcycles} is of the form
  $$
  (\theta^{\varepsilon_{1},n_{1}}_{v,x_{1}} \collapse{x_{1}}
  H_{1}) \collapse{v} \ldots \collapse{v}
  (\theta^{\varepsilon_{h},n_{h}}_{v,x_{h}} \collapse{x_{h}}
  H_{h})
  $$  
  %% $\collapse{v} \theta^{\varepsilon_{x},n_{x}}_{v,x} \collapse{x}
  %% H_{x}$ 
  if and only if for each distinct pair $A,B \in {\cal I}$ we
  have $A \cap B = \emptyset$.
\end{lemma}
\begin{proof}
  The condition is clearly necessary, since if $v$ is a glue point of
  a glue graph, then the patterns
  $$
  \xygraph{ %
    []*+{v}="v"
    -[rd]*+{}="b" 
    -[ld]*+{c}="c" 
    -[lu]*+{x}="x" -"v"
    "x"-[d]*+{} }
  \;\;\;\;
  \xygraph{ %
    []*+{v}="v"
    -[rd]*+{y}="y" 
    -[ld]*+{c}="c" 
    -[lu]*+{x}="x" -"v"
    "y"-[d]*+{} 
    "x"-[d]*+{}
  }
  \;\;\;\;
  \xygraph{ %
    []*+{v}="v"
    -[rd]*+{c}="b"  
    -[ll]*+{x}="x" -"v"
    "b"-"x"
    "b"-[d]*+{} 
    "x"-[d]*+{}
  }
  $$
  cannot arise. The first pattern illustrates $xE^{v} \cap S_{2}  \neq
  \emptyset$ for some $x \in S_{n2}$, the second $xE^{v} \cap
  yE^{v} \neq \emptyset$, for some $x,y \in S_{n2}$, and the third 
  $xE^{v} \cap S_{n2}  \neq \emptyset$ for some $x \in S_{n2}$.

  Conversely let us suppose that the family ${\cal I}$ is disjoint, so
  that these patterns do not arise. Let $x,y \in vE$ such that
  $\deg[G]{x} = \deg[G]{y} = 2$, so that $s(x),s(y) \in S_{2}$, and
  let $z,w \in S_{n2}$.

  (i) If there exists a symple path from $s(x)$ to $z$ which does not
  visit $v$, then we construct a symple cycle $v x s(x) \ldots zv$
  which, by condition \eqref{cond:shortcycles}, is of the form
  $vxs(x)zv$. This shows that $s(x) \in S_{2} \cap yE^{v} \neq
  \emptyset$, contradicting the hypothesis.

  (ii) If there exists a simple path from $z$ to $w$ which does not
  visit $v$, then we can construct a simple cycle $vz \ldots wv$
  which, by condition \eqref{cond:shortcycles}, is either of the form
  $v zu wv$ or of the form $vzwv$. Thus either $zE^{v} \cap wE^{v}
  \neq \emptyset$ or $S_{n2} \cap wE^{v} \neq \emptyset$, contradicting
  the hypothesis.
 
  (iii) Finally, let us suppose that $s(x)\neq s(y)$ and there exists
  a simple path $s(x)\ldots s(y)$ not visiting $v$.  Consider the path
  $vxs(x)\ldots s(y)yv$: because of condition
  \eqref{cond:shortcycles}, $x,s(x),s(y),y$ cannot be distinct.  If $x
  = s(y)$ then $y =s(x)$, by $\deg[G]{x} = \deg[G]{x} = 2$.  It
  follows that $s(x),s(y),v$ lie on a triangle.

  From this analysis, it follows that removing $v$ from $G$ disconnect
  elements of $S_{2} \cup S_{n2}$, up to some edges $\couple{x,y}$
  with $x,y \in S_{2}$.

  Thus for $w \in S_{2} \cup S_{n2}$ let $G_{w}$ be the connected
  component of $w$ in $G \setminus \set{v}$, and let $G_{w}^{v}$ be
  the subgraph of $G$ induced by $V_{G_{w}} \cup \set{v}$. If $w \in
  S_{n2}$ then $G_{w}^{v} = \theta^{1,0}_{v,w} \collapse{w} H$. If $w
  \in S_{2} \setminus vE$, then $G_{w}^{v} = \theta^{0,n}_{v,w}
  \collapse{w} H$, where $n = \card{\set{x \in vE|\,s(x) = w}}$.  If
  $w \in S_{2} \cap vE$, then $G_{w}^{v} = \theta^{1,n}_{v,w}
  \collapse{w} H$, where $n = \card{\set{x \in vE|\,s(x) = w}}$.  \qed
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

